Addressing Feature Suppression in Unsupervised Visual Representations

Contrastive learning is one of the fastest growing research areas in machine learning due to its ability to learn useful representations without labeled data. However, contrastive learning is susceptible to feature suppression, i.e., it may discard important information relevant to the task of interest, and learn irrelevant features. Past work has addressed this limitation via handcrafted data augmentations that eliminate irrelevant information. This approach however does not work across all datasets and tasks. Further, data augmentations fail in addressing feature suppression in multi-attribute classification when one attribute can suppress features relevant to other attributes. In this paper, we analyze the objective function of contrastive learning and formally prove that it is vulnerable to feature suppression. We then present predictive contrastive learning (PCL), a framework for learning unsupervised representations that are robust to feature suppression. The key idea is to force the learned representation to predict the input, and hence prevent it from discarding important information. Extensive experiments verify that PCL is robust to feature suppression and outperforms state-of-the-art contrastive learning methods on a variety of datasets and tasks.

==> source/ablation.tex <==
\subsection{Ablation Study on Reconstructive Tasks}
\label{sec:ablation}
\begin{table}[h]
\centering
\begin{tabular}{l |@{\hspace{0.2cm}} c| c @{\hspace{0.2cm}}  c @{\hspace{0.2cm}}c  @{\hspace{0.2cm}}c}\hline
  &  RF-MMD & \multicolumn{2}{c}{Colorful-Moving-MNIST}  \\
\hline
Recon. Tasks & Pose Err.   & \begin{tabular}{@{}c@{}}digit cls. \\ error rate\end{tabular} & \begin{tabular}{@{}c@{}}bkgd cls. \\ error rate\end{tabular}  &  \\
\hline
No Recon. & 80.5 & 85.1  & 51.5 \\
\hline
Colorization & N/A & 39.9 & 54.5 \\
Jigsaw Puzzle & N/A & 22.9 & 59.3\\
\hline
Autoencoder & 51.1  & 34.4 & 57.1 \\
Inpainting & 46.6 & 11.7 & 54.0 \\
\hline
\end{tabular}
\caption{Evaluation of different reconstructive tasks.}
\label{tab:ablation}
\end{table}


In \name, we choose the inpainting task for the reconstructive branch. However, other reconstructive tasks can be potentially used for the reconstructive branch. In this section, we evaluate the performance of \name~with different reconstructive tasks including inpainting, auto-encoder, colorization \cite{zhang2016colorful}, and Jigsaw Puzzle \cite{noroozi2016unsupervised}. Table \ref{tab:ablation} shows \name's performance using different reconstructive task on RF-based 3D pose estimation (RF-MMD) and Colorful-Moving-MNIST under the fixed feature extractor setting. As shown in the table, all reconstructive tasks significantly reduce errors in comparison to using contrastive learning without any reconstruction task.  The table also shows that inpaintaing compares favorably to other tasks and works across modalities. Hence, we use inpainting as the default reconstructive task  in IPCL. 


==> source/intro-1.tex <==
\section{Introduction}
The area of unsupervised or self-supervised representation learning is growing rapidly~\cite{he2020momentum,doersch2015unsupervised,ye2019unsupervised,hjelm2018learning,grill2020bootstrap,bachman2019learning,zhuang2019local,misra2020self,han2020memory}.
%pathak2016context,noroozi2016unsupervised,he2020momentum}. 
%~\cite{noroozi2016unsupervised,pathak2016context,gidaris2018unsupervised,oord2018representation,chen2020improved,he2020momentum,chen2020simple,chen2020big,ji2019invariant,sohn2016improved,icmlunsupervised,ye2019unsupervised}.  
It refers to learning data representations that capture potential labels of interest, and doing so without human supervision. Contrastive learning is increasingly considered as a standard and highly competitive method for unsupervised representation learning. Features learned with this method have been shown to generalize well to downstream tasks,  and in some cases surpass the performance of supervised models~\cite{oord2018representation,caron2020unsupervised,tschannen2019mutual,chen2020simple,chen2020big,chen2020improved}. 
 
Contrastive learning learns representations by contrasting positive samples against negative samples. During training, a data sample is chosen as an anchor (e.g., an image);  positive samples are chosen as different augmented versions of the anchor (e.g., randomly cropping and color distorting the image), whereas negative samples come from other samples in the dataset. 
 
Yet contrastive learning is vulnerable to shortcuts -- i.e., if simple features are contrastive enough to separate positive samples from negative samples, contrastive learning might learn such simple (or simpler) features even if irrelevant to the tasks of interest, and ignore other more relevant features. For example, the authors of \cite{chen2020simple} show that color distribution can be a shortcut to distinguish patches cropped from the same image, from patches from different images; yet such feature is not useful for object classification. Past work addresses this problem by designing handcrafted data augmentations to break such shortcuts, so that the network may learn the relevant information \cite{he2020momentum,chen2020simple,chen2020big,chen2020improved,chen2020intriguing}. 

However, it is not always possible to address shortcuts via data augmentation. 

\begin{figure}
\begin{center}
%\includegraphics[width=\linewidth]{pos-neg}
%\vspace{-15pt}
\begin{tabular}{ccc}
\includegraphics[width=0.14\textwidth]{rf.png} & \hspace*{-0.12in}
\label{fig:intro_rf}
\includegraphics[width=0.14\textwidth]{digit.jpg} & \hspace*{-0.12in}
\includegraphics[width=0.14\textwidth]{face.jpg}\\
{\footnotesize (a) Radio Signal} & \hspace*{-0.12in} {\footnotesize (b) Digit \& Bkgd} & \hspace*{-0.12in} {\footnotesize (c) Face Attribute}
\end{tabular}
\end{center}
%\vspace{-10pt}
\caption{\footnotesize{(a) Radio signals can have shortcuts that are hard to eliminate via handcrafted data augmentations. (b) In Colorful-MNIST \cite{tian2020makes}, the input has two types of information: digit and background object. But contrastive learning methods focus on the background object and ignore the digit. (c) Each image in FairFace \cite{karkkainen2019fairface} has multiple attributes such as age, gender, ethnicity, etc. Existing contrastive learning methods focus on ethnicity and partially ignore other attributes.}}
\label{fig:intro}
%\vspace{-11pt}
\end{figure}

Moreover, it is hard to design augmentations that generalize across different downstream tasks.
For example, the authors of \cite{tian2020makes} highlight the scenario in Fig.~\ref{fig:intro} (b), where each image shows a digit (from MNIST) on a randomly chosen background object (from STL-10).  They show that features related to background objects can create a shortcut that prevents contrastive learning from learning features related to digits. It is unclear how to design augmentations to learn features useful for digit classification, while keeping good performance on background object classification. A similar problem exists in the task of human face attribute classification, where each face image can be used in multiple downstream tasks including gender, age, and ethnicity classification (Fig.~\ref{fig:intro} (c)), but the features learned by contrastive learning can be biased to only one of the attributes (e.g., ethnicity) and show poor performance on other attributes (gender and age) (Sec. \ref{sec:rgb}). In this case, it is hard to come up with data augmentations that eliminate the shortcut attribute without harming the corresponding classification task. 

To solve this problem, we propose reconstructive contrastive learning (\name), a new unsupervised learning framework that works across different modalities and tasks. The key idea underlying \name~is to learn representations using contrastive and reconstructive learning simultaneously. We use the term reconstructive learning to refer to tasks that force the representation to reconstruct the input, such as inpainting, colorization, or autoencoding. Such tasks counter the effect of shortcuts because they force the learned features to retain the information in the input. Once combined with reconstructive learning,  contrastive learning ensures that all useful features (not just the shortcut features) are closely mapped in the embedding space for positive samples, and stay distant for negative samples. Thus, reconstructive learning maximizes the useful information in the representation, whereas contrastive learning orders the information in the embedding space to make it easy for a simple classifier to slice the embedding space to satisfy a desired task. 

%The key idea underlying IPCL is to ensure that even when the data has potential shortcuts, the representation will learn features about all types of semantic information in the data (digit and background object), and contrastive learning will ensure that all of those features (not just the shortcut features) are closely mapped in the embedding space for positive samples, and stay distant for negative samples.  To ensure that these properties are satisfied, IPCL augments contrastive learning with an auxiliary task that uses the learned representation to restore randomly cropped patches in the anchor sample. By doing so, IPCL ensures that the learned representation summarizes all useful information in the input, but also enjoys contrastive properties. 


%We apply the IPCL framework to both RGB-based and RF-based tasks, designing neural network models appropriate for those modalities.   

We evaluate \name~and compare it with state-of-the-art contrastive learning baselines on four different RGB datasets: ImageNet-100 \cite{tian2019contrastive},  MPII \cite{andriluka20142d}, Colorful-MNIST \cite{tian2020makes}, and FairFace \cite{karkkainen2019fairface}, and three RF-based sensing tasks: 3D pose estimation, human action recognition, and person re-identification. For all tasks, \name~achieves superior performance and outperforms the state-of-the-art baselines by large margins, demonstrating its robustness against shortcuts and its ability to learn general features for different downstream tasks. 

To summarize, this paper makes the following contributions:
\begin{Itemize}
	\item \blue{It proves that the global minimum of infoNCE loss at a lower feature dimension indicates a local minimum or saddle point of infoNCE loss at a higher feature dimension, which gives a theoretical explanation to why contrastive learning is vulnerable to shortcut.}
    \item It introduces \name, \blue{a} self-supervised learning framework that integrates contrastive and reconstructive learning to automatically avoid shortcuts and provide a representation that supports multiple different downstream tasks.     
    \item It empirically shows the negative impact shortcuts have on contrastive learning and demonstrates that \name~outperforms SOTA contrastive learning in its ability to avoid shortcuts and learn general representations that support multiple downstream tasks.
\end{Itemize}



%\begin{Itemize}
%\item 

%\item 
%{\it (a) Results on RGB Data:}
%we evaluate IPCL on four different RGB datasets: Colorful-MNIST \cite{tian2020makes}, FairFace \cite{karkkainen2019fairface}, MPII \cite{andriluka20142d} and ImageNet-100 \cite{tian2019contrastive}. On Colorful-MNIST, in comparison to the contrastive learning baselines, the \name~representation has 72\% higher accuracy on digit classification and comparable performance on background classification. On FairFace, \name~improves over baselines performance on age and gender classification by 5.7\% and 8.6\% respectively, while keeping comparable performance on ethnicity classification (61.2\% vs. 62.3\%). On MPII, \name~outperforms baselines by 3.7 PCKh under fixed feature encoder setting and 0.7 PCKh under fine-tuning setting. And on ImageNet-100, IPCL is much more robust to the choice of image augmentations than contrastive methods. It achieves comparable results as state-of-the-art contrastive learning methods under full sets of augmentations (\red{80.5\%} vs. \red{81.2\%}), and keeps displaying good performance when only a subset of augmentations are applied while the performance of other contrastive baselines drops significantly (\red{74.2\%} vs. \red{67.2}\% when only applying random crop as augmentation).
%
%{\it (a) Results on RF Data:}
%We evaluate IPCL on three real-world RF-based sensing tasks: 3D pose estimation, human action recognition, and person re-identification. 
%The results show that IPCL outperforms all contrastive learning baselines on all tasks.  In comparison to the best performing contrastive learning baseline, the IPCL representation improves performance by 30.6 mm, 81.4 mAP, and 24.5 mAP on the tasks of pose estimation, action recognition, and person re-id respectively.  
%%Further, initializing supervised learning with the IPCL representation improves performance for all three tasks, confirming that self-supervision is beneficial for learning from non-interpretable data. 
%Interestingly, the representations learned by the contrastive learning baselines perform worse than random features on pose estimation and action recognition. This shows that contrastive learning converged on a shortcut, and discarded key information necessary for these two  tasks.  

%\red{We also empirically show the complexity of reasoning about shortcuts even in RGB images, and how IPCL overcomes this complexity.}

%Our method can achieve 11.7\% error rate on digit classification and 54.0\% error rate on background object classification, while all other contrastive learning baselines have near-random error rate on digit classification ($\sim$90\%) and have comparable error rates to IPCL on background object classification (51\% to 64\%). The second dataset is FairFace~\cite{karkkainen2019fairface}, where we show that IPCL is more effective than state-of-the-art contrastive learning at learning a single representation that works for multiple downstream classification tasks based on race, gender and age. \name~outperforms SimCLR on age and gender classification by 5.7\% and 8.6\% in error rate, and achieves comparable results as SimCLR on ethnicity classification (38.8\% vs. 37.7\% error rate).

%\end{Itemize}

